A Mixed-Methods Study of Open-Source Software Maintainers On Vulnerability Management and Platform Security Features

In open-source software (OSS), software vulnerabilities have significantly increased. Although researchers have investigated the perspectives of vulnerability reporters and OSS contributor security practices, understanding the perspectives of OSS maintainers on vulnerability management and platform security features is currently understudied. In this paper, we investigate the perspectives of OSS maintainers who maintain projects listed in the GitHub Advisory Database. We explore this area by conducting two studies: identifying aspects through a listing survey ($n_1=80$) and gathering insights from semi-structured interviews ($n_2=22$). Of the 37 identified aspects, we find that supply chain mistrust and lack of automation for vulnerability management are the most challenging, and barriers to adopting platform security features include a lack of awareness and the perception that they are not necessary. Surprisingly, we find that despite being previously vulnerable, some maintainers still allow public vulnerability reporting, or ignore reports altogether. Based on our findings, we discuss implications for OSS platforms and how the research community can better support OSS vulnerability management efforts.

==> content/original2.tex <==

 \begin{table*}[ht!]
 \centering
 \begin{adjustbox}{width=\textwidth}
 %\begin{tabular}{p{0.15cm}p{3.7cm}p{7.79cm}rrl}
 %\begin{tabular}{llllp{2.14cm}rl}
 \begin{tabular}{p{0.15cm}lllp{2.68cm}rl}
 \toprule
 %\midrule
  & \multicolumn{1}{l}{\textbf{Factors and tooling}} & \multicolumn{1}{l}{\textbf{Description}} & \multicolumn{1}{l}{\diffadd{\textbf{F\#}}} & \multicolumn{1}{l}{\textbf{RW}} & \multicolumn{1}{r}{\textbf{L}} & \multicolumn{1}{l}{\textbf{I}} \\
 \midrule
 \parbox[t]{1mm}{\multirow{8}{*}{\rotatebox[origin=c]{90}{\textbf{Current practices}}}}
   & \textbf{Email or mailing list} & Uses a private email or mailing list for vulnerabilities. & F1 & \cite{wermke2022qual-OSSP,lee2017understanding}  & 50 & 11 \\
   %%\cmidrule(lr){2-6}
   & \cellcolor{grey1}\textbf{Proactive disclosure} & \cellcolor{grey1}Established disclosure process after a vulnerability patch. & \cellcolor{grey1}F2 & \cellcolor{grey1}\cite{wermke2022qual-OSSP} & \cellcolor{grey1}46 & \cellcolor{grey1}7 \\
   & \textbf{Security policy} & Instructs users how to report vulnerabilities. & F3 & \cite{wermke2022qual-OSSP} & 37 & 10 \\
   %%\cmidrule(lr){2-6}
   & \cellcolor{grey1}\textbf{GitHub private reporting} & \cellcolor{grey1}A built-in feature for privately reporting vulnerabilities. & \cellcolor{grey1}F4 & \cellcolor{grey1} & \cellcolor{grey1}20 & \cellcolor{grey1}9 \\
   %%\cmidrule(lr){2-6}
   & \textbf{Automation tooling} & E.g., Dependabot, code scanning, secret scanning. & F5 & \cite{onsori2024quantifying,dietrich2023security,he2023automating,mohayeji2023investigating,alfadel2021use,mirhosseini2017can} & 16 & 12 \\
   %%\cmidrule(lr){2-6}
   & \cellcolor{grey1}\textbf{GitHub Issues} & \cellcolor{grey1}Vulnerabilities are reported publicly with GitHub Issues. & \cellcolor{grey1}F6 & \cellcolor{grey1}\cite{preceptionofoss} & \cellcolor{grey1}9 & \cellcolor{grey1}6 \\
   %%\cmidrule(lr){2-6}
   & \textbf{External tooling} & Utilizes tooling or reports outside of GitHub. & F7 & \cite{he2023automating,wermke2022qual-OSSP,fischer2023effectiveness}  & 3 & 2 \\
   %%\cmidrule(lr){2-6}
   & \cellcolor{grey1}\textbf{Ignores vulnerabilties} & \cellcolor{grey1}Ignores vulnerability reports or does nothing in response. & \cellcolor{grey1}F8 & \cellcolor{grey1} & \cellcolor{grey1}2 & \cellcolor{grey1}-- \\
  \midrule
 \parbox[t]{1mm}{\multirow{9}{*}{\rotatebox[origin=c]{90}{\textbf{General challenges}}}}
   & \textbf{Supply chain trust} & E.g., waiting for upstream dependencies to deploy a fix. & F9 & \cite{alomar2020you,wermke2022qual-OSSP,dabbish2012social,okafor2022soksssc,fourne2023s} & 36 & 6 \\
   & \cellcolor{grey1}\textbf{Lack of understanding} & \cellcolor{grey1}E.g., knowledge gaps, how to start developing a patch. & \cellcolor{grey1}F10 & \cellcolor{grey1}\cite{alomar2020you,anon2025deepdive} & \cellcolor{grey1}35 & \cellcolor{grey1}12 \\
   & \textbf{Lack of time} & Balancing vulnerability priority with other OSS tasks. & F11 & \cite{lawsonfeel,wermke2022qual-OSSP,anon2025deepdive} & 25 & 9 \\
   & \cellcolor{grey1}\textbf{Lack of resources} & \cellcolor{grey1}E.g., \textit{``I do almost everything myself''} (P4). & \cellcolor{grey1}F12 & \cellcolor{grey1}\cite{wermke2022qual-OSSP,canfora2020process} & \cellcolor{grey1}23 & \cellcolor{grey1}11 \\
   & \textbf{CVE relationships} & Negative experiences with CVE-assigned vulnerabilities. & F13 & & 8 & 9 \\
   & \cellcolor{grey1}\textbf{Lack of procedure} & \cellcolor{grey1}Maintainers are not sure how to deal with vulnerabilities. & \cellcolor{grey1}F14 & \cellcolor{grey1}\cite{wermke2022qual-OSSP} & \cellcolor{grey1}7 & \cellcolor{grey1}5 \\
   & \textbf{Disclosure coordination} & How to reach out to all users and what to disclose. & F15 & \cite{alomar2020you} & 7 & 4 \\
   & \cellcolor{grey1}\textbf{Negative attitudes} & \cellcolor{grey1}Past negative interactions with reporters or companies. & \cellcolor{grey1}F16 & \cellcolor{grey1}\cite{miller2022did,raman2020burnout,windowshit,nodeleave,lawsonfeel,destefanis2016software} & \cellcolor{grey1}6 & \cellcolor{grey1}9 \\
 \midrule
   \parbox[t]{1mm}{\multirow{8}{*}{\rotatebox[origin=c]{90}{\textbf{PSF challenges}}}}
   & \textbf{Not enough automation} & More automation needed in PSF functionality. & F17 & \cite{kabadi2023apr,bui2024apr} & 39 & 11 \\
   &  \cellcolor{grey1}\textbf{Too much noise} & \cellcolor{grey1}E.g., too many false positives. & \cellcolor{grey1}F18 & \cellcolor{grey1}\cite{wermke2022qual-OSSP,wedyan2009effectiveness,he2023automating,mirhosseini2017can,wessel2021don,wessel2022bots,brown2019sorry,zampetti2017open} & \cellcolor{grey1}24 & \cellcolor{grey1}10 \\
   & \textbf{Vulnerability scoring} & E.g., having a hard time calculating CVSS scores. & F19 & & 21 & 9 \\
   & \cellcolor{grey1}\textbf{CI processes are missing} & \cellcolor{grey1}GitHub Actions \& tests are not available in private forks. & \cellcolor{grey1}F20 & \cellcolor{grey1} & \cellcolor{grey1}8 & \cellcolor{grey1}7 \\
   & \textbf{Broken tests \& builds} & Failing builds \& tests after vulnerability patch is applied. & F21 & \cite{zampetti2017open,rausch2017empirical,mirhosseini2017can,brown2019sorry} & 6 & 7 \\
   & \cellcolor{grey1}\textbf{Cluttered notifications} & \cellcolor{grey1}E.g., vulnerable dependencies presentation is cluttered. & \cellcolor{grey1}F22 & \cellcolor{grey1} & \cellcolor{grey1}4 & \cellcolor{grey1}4 \\
   & \textbf{Too much manual setup} & E.g., manually enabling PSFs on all projects. & F23 & & 3 & 3 \\
  \midrule
   \parbox[t]{1mm}{\multirow{7}{*}{\rotatebox[origin=c]{90}{\textbf{PSF barriers}}}}
   & \cellcolor{grey1}\textbf{Lack of awareness} & \cellcolor{grey1}E.g., not knowing about private vulnerability reporting. & \cellcolor{grey1}F24 & \cellcolor{grey1}\cite{ayala2024secfeat} & \cellcolor{grey1}33 & \cellcolor{grey1}12 \\
   & \textbf{Complex to set up or use} & PSFs are too complex for maintainers with limited time. & F25 & & 26 & 7 \\
   & \cellcolor{grey1}\textbf{They are unnecessary} & \cellcolor{grey1}Perception that using PSFs is not needed. & \cellcolor{grey1}F26 & \cellcolor{grey1} & \cellcolor{grey1}23 & \cellcolor{grey1}6 \\
   & \textbf{Reputation concerns} & Past vulnerabilities reflect a negative project reputation. & F27 & & 11 & 4 \\
   & \cellcolor{grey1}\textbf{Bad UI presentation} & \cellcolor{grey1}Hard to find or hidden, \textit{``second-class features''} (P10). & \cellcolor{grey1}F28 & \cellcolor{grey1}\cite{danilova2020one,johnson2013don,fischer2023effectiveness} & \cellcolor{grey1}8 & \cellcolor{grey1}6 \\
   & \textbf{Lack of motivation} & Feeling burned out from other OSS tasks. & F29 & \cite{raman2020burnout, openssfwgs, linåker2024sustaining, amit2024motivation,lawsonfeel} & 5 & 4 \\
   & \cellcolor{grey1}\textbf{Not sure what they do} & \cellcolor{grey1}Unsure of PSFs' functionality, benefits, etc. & \cellcolor{grey1}F30 & \cellcolor{grey1} & \cellcolor{grey1}4 & \cellcolor{grey1}2 \\
  \midrule
   \parbox[t]{1mm}{\multirow{7}{*}{\rotatebox[origin=c]{90}{\textbf{Maintainer wants}}}}
   & \textbf{Assisted triaging} & Automation for impact analysis, patch development, etc. & F31 & \cite{kabadi2023apr,bui2024apr,wessel2022bots} & 39 & 9 \\   
   & \cellcolor{grey1}\textbf{Assisted PSF setup} & \cellcolor{grey1}More guidance for the PSF setup process. & \cellcolor{grey1}F32 & \cellcolor{grey1} & \cellcolor{grey1}37 & \cellcolor{grey1}10 \\
   & \textbf{Security-specific funding} & Opportunities for funding OSS security efforts. & F33 & \cite{wermke2022qual-OSSP} & 32 & 7 \\
   & \cellcolor{grey1}\textbf{User-friendly resources} & \cellcolor{grey1}Tailored for those without a security background. & \cellcolor{grey1}F34 & \cellcolor{grey1} & \cellcolor{grey1}17 & \cellcolor{grey1}8 \\
%   & \textbf{Tooling recommendations} & The ability to provide feedback and make report adjustments. & & &  \\
   & \textbf{Gamification for projects} & E.g., a green shield for projects with proper PSFs set up. & F35 & \cite{moldon2021gamification,trockman2018adding,dabbish2012social} & 13 & 6 \\
   & \cellcolor{grey1}\textbf{PSF checklist} & \cellcolor{grey1}To-do list for enabling easily configurable PSFs. & \cellcolor{grey1}F36 & \cellcolor{grey1} & \cellcolor{grey1}15 & \cellcolor{grey1}3 \\   
   & \textbf{Nudges or reminders} & Nudges reminding maintainers to consider using PSFs. & F37 & & 12 & 5 \\
%   & \rowcolor{grey1} \textbf{Dependency inspection} & Comments and messaging are available during the review process. &  & &  \\
%   & \rowcolor{grey1} \textbf{Auto-merge configurations} & Streamlined and assisted process of creating CVEs. & & &  \\
  \bottomrule
 \end{tabular}
 \end{adjustbox}
 \caption{\codenums factors and tooling codes, shortened to preserve space, identified from the listing survey study and interview study divided into five categories as a result of software vulnerability management efforts. Acronyms listed represent, respectively: platform security features (\textbf{PSF}), existing related work (\textbf{RW}), the number of listing (\textbf{L}) survey study mentions ($n_1=80$), and the number of interview (\textbf{I}) study mentions  ($n_2=22$). The extended table without omitted codes can be found in our artifact~\cite{icse25repo}.}
    \label{tab:bigasstable}
 %\end{centering}
 \end{table*}


==> content/table_nocolors.tex <==
 \begin{table*}[ht!]
 \centering
 %\begin{adjustbox}{width=\textwidth}
 \begin{tabular}{cp{3.695cm}p{7.79cm}lp{2.14cm}rl}
 \toprule
 %\midrule
  & \multicolumn{1}{l}{\textbf{Factors and tooling}} & \multicolumn{1}{l}{\textbf{Description}} & \multicolumn{1}{l}{\textbf{F\#}} & \multicolumn{1}{l}{\textbf{RW}} & \multicolumn{1}{r}{\textbf{L}} & \multicolumn{1}{l}{\textbf{I}} \\
 \midrule
 \parbox[t]{1mm}{\multirow{8}{*}{\rotatebox[origin=c]{90}{\textbf{Current practices}}}}
   & \textbf{Email or mailing list} & Have a private email or mailing list for vulnerabilities. & F1 & \cite{wermke2022qual-OSSP,lee2017understanding}  & 50 & 11 \\
   %%\cmidrule(lr){2-6}
   & \cellcolor{grey1}\textbf{Proactive disclosure} & \cellcolor{grey1}Established disclosure process after a vulnerability patch. & \cellcolor{grey1}F2 & \cellcolor{grey1}\cite{wermke2022qual-OSSP} & \cellcolor{grey1}46 & \cellcolor{grey1}7 \\
   & \textbf{Security policy} & Instructs users how to report vulnerabilities. & F3 & \cite{wermke2022qual-OSSP} & 37 & 10 \\
   %%\cmidrule(lr){2-6}
   & \cellcolor{grey1}\textbf{GitHub private reporting} & \cellcolor{grey1}A built-in feature for privately reporting vulnerabilities. & \cellcolor{grey1}F4 & \cellcolor{grey1} & \cellcolor{grey1}20 & \cellcolor{grey1}9 \\
   %%\cmidrule(lr){2-6}
   & \textbf{Automation tooling} & E.g., Dependabot, code scanning, secret scanning. & F5 & \cite{onsori2024quantifying,dietrich2023security,he2023automating,mohayeji2023investigating,alfadel2021use,mirhosseini2017can} & 16 & 12 \\
   %%\cmidrule(lr){2-6}
   & \cellcolor{grey1}\textbf{GitHub Issues} & \cellcolor{grey1}Vulnerabilities are reported publicly with GitHub Issues. & \cellcolor{grey1}F6 & \cellcolor{grey1}\cite{preceptionofoss} & \cellcolor{grey1}9 & \cellcolor{grey1}6 \\
   %%\cmidrule(lr){2-6}
   & \textbf{External tooling} & Utilizes tooling or reports outside of GitHub. & F7 & \cite{he2023automating,wermke2022qual-OSSP,fischer2023effectiveness}  & 3 & 2 \\
   %%\cmidrule(lr){2-6}
   & \cellcolor{grey1}\textbf{Ignores vulnerabilties} & \cellcolor{grey1}Ignores vulnerability reports or does nothing in response. & \cellcolor{grey1}F8 & \cellcolor{grey1} & \cellcolor{grey1}2 & \cellcolor{grey1}-- \\
  \midrule
 \parbox[t]{1mm}{\multirow{8}{*}{\rotatebox[origin=c]{90}{\textbf{General challenges}}}}
   & \textbf{Supply chain trust} & E.g., waiting for upstream dependencies to deploy a fix. & F9 & \cite{alomar2020you,wermke2022qual-OSSP,dabbish2012social,okafor2022soksssc,fourne2023s} & 36 & 6 \\
   & \cellcolor{grey1}\textbf{Lack of understanding} & \cellcolor{grey1}E.g., knowledge gaps, how to start developing a patch. & \cellcolor{grey1}F10 & \cellcolor{grey1}\cite{alomar2020you,anon2025deepdive} & \cellcolor{grey1}35 & \cellcolor{grey1}12 \\
   & \textbf{Lack of time} & Balancing vulnerability priority with other OSS tasks. & F11 & \cite{lawsonfeel,wermke2022qual-OSSP,anon2025deepdive} & 25 & 9 \\
   & \cellcolor{grey1}\textbf{Lack of resources} & \cellcolor{grey1}E.g., \textit{``I do almost everything myself''} (P4). & \cellcolor{grey1}F12 & \cellcolor{grey1}\cite{wermke2022qual-OSSP,canfora2020process} & \cellcolor{grey1}23 & \cellcolor{grey1}11 \\
   & \textbf{CVE relationships} & Negative experiences with CVE-assigned vulnerabilities. & F13 & & 8 & 9 \\
   & \cellcolor{grey1}\textbf{Lack of procedure} & \cellcolor{grey1}Maintainers are not sure how to deal with vulnerabilities. & \cellcolor{grey1}F14 & \cellcolor{grey1}\cite{wermke2022qual-OSSP} & \cellcolor{grey1}7 & \cellcolor{grey1}5 \\
   & \textbf{Disclosure coordination} & How to reach out to all users and what to disclose. & F15 & \cite{alomar2020you} & 7 & 4 \\
   & \cellcolor{grey1}\textbf{Negative attitudes} & \cellcolor{grey1}Past negative interactions with reporters or companies. & \cellcolor{grey1}F16 & \cellcolor{grey1}\cite{miller2022did,raman2020burnout,windowshit,nodeleave,lawsonfeel,destefanis2016software} & \cellcolor{grey1}6 & \cellcolor{grey1}9 \\
 \midrule
   \parbox[t]{1mm}{\multirow{7}{*}{\rotatebox[origin=c]{90}{\textbf{PSF challenges}}}}
   & \textbf{Not enough automation} & More automation needed in PSF functionality. & F17 & \cite{kabadi2023apr,bui2024apr} & 39 & 11 \\
   &  \cellcolor{grey1}\textbf{Too much noise} & \cellcolor{grey1}E.g., too many false positives. & \cellcolor{grey1}F18 & \cellcolor{grey1}\cite{wermke2022qual-OSSP,wedyan2009effectiveness,he2023automating,mirhosseini2017can,wessel2021don,wessel2022bots,brown2019sorry,zampetti2017open} & \cellcolor{grey1}24 & \cellcolor{grey1}10 \\
   & \textbf{Vulnerability scoring} & E.g., having a hard time calculating CVSS scores. & F19 & & 21 & 9 \\
   & \cellcolor{grey1}\textbf{CI processes are missing} & \cellcolor{grey1}GitHub Actions \& tests are not available in private forks. & \cellcolor{grey1}F20 & \cellcolor{grey1} & \cellcolor{grey1}8 & \cellcolor{grey1}7 \\
   & \textbf{Broken tests \& builds} & Failing builds \& tests after vulnerability patch is applied. & F21 & \cite{zampetti2017open,rausch2017empirical,mirhosseini2017can,brown2019sorry} & 6 & 7 \\
   & \cellcolor{grey1}\textbf{Cluttered notifications} & \cellcolor{grey1}E.g., vulnerable dependencies presentation is cluttered. & \cellcolor{grey1}F22 & \cellcolor{grey1} & \cellcolor{grey1}4 & \cellcolor{grey1}4 \\
   & \textbf{Too much manual setup} & E.g., manually enabling PSFs on all projects. & F23 & & 3 & 3 \\
  \midrule
   \parbox[t]{1mm}{\multirow{7}{*}{\rotatebox[origin=c]{90}{\textbf{PSF barriers}}}}
   & \cellcolor{grey1}\textbf{Lack of awareness} & \cellcolor{grey1}E.g., not knowing about private vulnerability reporting. & \cellcolor{grey1}F24 & \cellcolor{grey1}\cite{ayala2024secfeat} & \cellcolor{grey1}33 & \cellcolor{grey1}12 \\
   & \textbf{Complex to set up or use} & PSFs are too complex for maintainers with limited time. & F25 & & 26 & 7 \\
   & \cellcolor{grey1}\textbf{They are unnecessary} & \cellcolor{grey1}Perception that using PSFs is not needed. & \cellcolor{grey1}F26 & \cellcolor{grey1} & \cellcolor{grey1}23 & \cellcolor{grey1}6 \\
   & \textbf{Reputation concerns} & Past vulnerabilities reflect a negative project reputation. & F27 & & 11 & 4 \\
   & \cellcolor{grey1}\textbf{Bad UI presentation} & \cellcolor{grey1}Hard to find or hidden, \textit{``second-class features''} (P10). & \cellcolor{grey1}F28 & \cellcolor{grey1}\cite{danilova2020one,johnson2013don,fischer2023effectiveness} & \cellcolor{grey1}8 & \cellcolor{grey1}6 \\
   & \textbf{Lack of motivation} & Feeling burned out from other OSS tasks. & F29 & \cite{raman2020burnout, openssfwgs, linåker2024sustaining, amit2024motivation,lawsonfeel} & 5 & 4 \\
   & \cellcolor{grey1}\textbf{Not sure what they do} & \cellcolor{grey1}Unsure of PSFs' functionality, benefits, etc. & \cellcolor{grey1}F30 & \cellcolor{grey1} & \cellcolor{grey1}4 & \cellcolor{grey1}2 \\
  \midrule
   \parbox[t]{1mm}{\multirow{7}{*}{\rotatebox[origin=c]{90}{\textbf{Maintainer wants}}}}
   & \textbf{Assisted triaging} & Automation for impact analysis, patch development, etc. & F31 & \cite{kabadi2023apr,bui2024apr,wessel2022bots} & 39 & 9 \\   
   & \cellcolor{grey1}\textbf{Assisted PSF setup} & \cellcolor{grey1}More guidance for the PSF setup process. & \cellcolor{grey1}F32 & \cellcolor{grey1} & \cellcolor{grey1}37 & \cellcolor{grey1}10 \\
   & \textbf{Security-specific funding} & Opportunities for funding OSS security efforts. & F33 & \cite{wermke2022qual-OSSP} & 32 & 7 \\
   & \cellcolor{grey1}\textbf{User-friendly resources} & \cellcolor{grey1}Tailored for those without a security background. & \cellcolor{grey1}F34 & \cellcolor{grey1} & \cellcolor{grey1}17 & \cellcolor{grey1}8 \\
%   & \textbf{Tooling recommendations} & The ability to provide feedback and make report adjustments. & & &  \\
   & \textbf{Gamification for projects} & E.g., a green shield for projects with proper PSFs set up. & F35 & \cite{moldon2021gamification,trockman2018adding,dabbish2012social} & 13 & 6 \\
   & \cellcolor{grey1}\textbf{PSF checklist} & \cellcolor{grey1}To-do list for enabling easily configurable PSFs. & \cellcolor{grey1}F36 & \cellcolor{grey1} & \cellcolor{grey1}15 & \cellcolor{grey1}3 \\   
   & \textbf{Nudges or reminders} & Nudges reminding maintainers to consider using PSFs. & F37 & & 12 & 5 \\
%   &   \textbf{Dependency inspection} & Comments and messaging are available during the review process. &  & &  \\
%   &   \textbf{Auto-merge configurations} & Streamlined and assisted process of creating CVEs. & & &  \\
  \bottomrule
 \end{tabular}
 %\end{adjustbox}
 \caption{\codenums factors and tooling codes, shortened to preserve space, identified from the listing survey study and interview study divided into five categories as a result of software vulnerability management efforts. Acronyms listed represent, respectively: platform security features (\textbf{PSF}), existing related work (\textbf{RW}), the number of listing (\textbf{L}) survey study mentions ($n_1=80$), and the number of interview (\textbf{I}) study mentions  ($n_2=22$). The extended table without omitted codes can be found in our artifact~\cite{icse25repo}.}
    \label{tab:bigasstable}
 %\end{centering}
 \end{table*}

==> content/table_original.tex <==

 \begin{table*}[ht!]
 \centering
 \begin{adjustbox}{width=\textwidth}
 %\begin{tabular}{p{0.15cm}p{3.7cm}p{7.79cm}rrl}
 \begin{tabular}{lllrrl}
 \toprule
 %\midrule
 & \multicolumn{1}{l}{\textbf{Factors and tooling}} & \multicolumn{1}{l}{\textbf{Description}} & \multicolumn{1}{r}{\textbf{RW}} & \multicolumn{1}{r}{\textbf{L}} & \multicolumn{1}{l}{\textbf{I}} \\
 \midrule
 \parbox[t]{1mm}{\multirow{8}{*}{\rotatebox[origin=c]{90}{\textbf{Current practices}}}}
   & \textbf{Email or mailing list} & A private email or mailing list for vulnerabilities. & \cite{wermke2022qual-OSSP,lee2017understanding}  & 50 & 11 \\
   & \cellcolor{grey1}\textbf{Proactive disclosure} & \cellcolor{grey1}Established disclosure process after a vulnerability patch. & \cellcolor{grey1}\cite{wermke2022qual-OSSP} & \cellcolor{grey1}46 & \cellcolor{grey1}7 \\
   & \textbf{Security policy} & Instructs users how to report vulnerabilities. & \cite{wermke2022qual-OSSP} & 37 & 10 \\
   & \rowcolor{grey1} \textbf{GitHub private reporting} & A built-in feature for privately reporting vulnerabilities. & & 20 & 9 \\
   & \textbf{Automation tooling} & E.g., Dependabot, code scanning, secret scanning. & \cite{onsori2024quantifying,dietrich2023security,he2023automating,mohayeji2023investigating,alfadel2021use,mirhosseini2017can} & 16 & 12 \\
   & \rowcolor{grey1} \textbf{GitHub Issues} & Vulnerabilities are reported publicly with GitHub Issues. &\cite{preceptionofoss} & 9 & 6 \\
   & \textbf{External tooling} & Utilizes tooling or reports outside of GitHub. & \cite{he2023automating,wermke2022qual-OSSP,fischer2023effectiveness}  & 3 & 2 \\
   & \rowcolor{grey1} \textbf{Ignores vulnerabilties} & Ignores vulnerability reports or does nothing in response. &  & 2 & -- \\
  \midrule
 \parbox[t]{1mm}{\multirow{8}{*}{\rotatebox[origin=c]{90}{\textbf{General challenges}}}}
   & \textbf{Supply chain trust} & E.g., waiting for upstream dependencies to deploy a fix. & \cite{alomar2020you,wermke2022qual-OSSP,dabbish2012social,okafor2022soksssc,fourne2023s} & 36 & 6 \\
   & \rowcolor{grey1} \textbf{Lack of understanding} & E.g., knowledge gaps, how to start developing a patch. & \cite{alomar2020you,anon2025deepdive} & 35 & 12 \\
   & \textbf{Lack of time} & Balancing vulnerability priority with other OSS tasks. & \cite{lawsonfeel,wermke2022qual-OSSP,anon2025deepdive} & 25 & 9 \\
   & \rowcolor{grey1} \textbf{Lack of resources} & E.g., \textit{``I do almost everything myself''} (P4). & \cite{wermke2022qual-OSSP,canfora2020process}  & 23 & 11 \\
   & \textbf{CVE relationships} & Negative experiences with CVE-assigned vulnerabilities. & & 8 & 9 \\
   & \rowcolor{grey1} \textbf{Lack of procedure} & Maintainers are not sure how to deal with vulnerabilities. & \cite{wermke2022qual-OSSP} & 7 & 5 \\
   & \textbf{Disclosure coordination} & How to reach out to all users and what to disclose. & \cite{alomar2020you} & 7 & 4 \\
   & \rowcolor{grey1} \textbf{Negative attitudes} & Past negative interactions with reporters or companies. & \cite{miller2022did,raman2020burnout,windowshit,nodeleave,lawsonfeel,destefanis2016software} & 6 & 9 \\
 \midrule
   \parbox[t]{1mm}{\multirow{7}{*}{\rotatebox[origin=c]{90}{\textbf{PSF challenges}}}}
   & \textbf{Not enough automation} & More automation needed in PSF functionality. & \cite{kabadi2023apr,bui2024apr} & 39 & 11 \\
   & \rowcolor{grey1} \textbf{Too much noise} & E.g., too many false positives. & \cite{wermke2022qual-OSSP,wedyan2009effectiveness,he2023automating,mirhosseini2017can,wessel2021don,wessel2022bots,brown2019sorry,zampetti2017open} & 24 & 10 \\
   & \textbf{Vulnerability scoring} & E.g., having a hard time calculating CVSS scores. & & 21 & 9 \\
   & \rowcolor{grey1} \textbf{CI processes are missing} & GitHub Actions \& tests are not available in private forks. & & 8 & 7 \\
   & \textbf{Broken tests \& builds} & Failing builds \& tests after vulnerability patch s applied. & \cite{zampetti2017open,rausch2017empirical,mirhosseini2017can,brown2019sorry} & 6 & 7 \\
   & \rowcolor{grey1} \textbf{Cluttered notifications} & E.g., vulnerable dependencies presentation is cluttered. & & 4 & 4 \\
   & \textbf{Too much manual setup} & E.g., manually enabling PSFs on all projects. & & 3 & 3 \\
  \midrule
   \parbox[t]{1mm}{\multirow{7}{*}{\rotatebox[origin=c]{90}{\textbf{PSF barriers}}}}
   & \rowcolor{grey1} \textbf{Lack of awareness} & E.g., not knowing about private vulnerability reporting. & \cite{ayala2024secfeat} & 33 & 12 \\
   & \textbf{Complex to set up or use} & PSFs are too complex for maintainers with limited time. & & 26 & 7 \\
   & \rowcolor{grey1} \textbf{They are unnecessary} & Perception that using PSFs is not needed. & & 23 & 6 \\
   & \textbf{Reputation concerns} & Past vulnerabilities reflects a negative project reputation. & & 11 & 4 \\
   & \rowcolor{grey1} \textbf{Bad UI presentation} & Hard to find or hidden, \textit{``second-class features''} (P10). & \cite{danilova2020one,johnson2013don,fischer2023effectiveness} & 8 & 6 \\
   & \textbf{Lack of motivation} & Feeling burned out from other OSS tasks. & \cite{raman2020burnout, openssfwgs, linåker2024sustaining, amit2024motivation,lawsonfeel} & 5 & 4 \\
   & \rowcolor{grey1} \textbf{Not sure what they do} & Unsure of PSFs' functionality, benefits, etc. & & 4 & 2 \\
  \midrule
   \parbox[t]{1mm}{\multirow{7}{*}{\rotatebox[origin=c]{90}{\textbf{Maintainer wants}}}}
   & \textbf{Assisted triaging} & Automation for impact analysis, patch development, etc. & \cite{kabadi2023apr,bui2024apr,wessel2022bots} & 39 & 9 \\   
   & \rowcolor{grey1} \textbf{Assisted PSF setup} & More guidance for the PSF setup process. & & 37 & 10 \\
   & \textbf{Security-specific funding} & Opportunities for funding OSS security efforts. & \cite{wermke2022qual-OSSP} & 32 & 7 \\
   & \rowcolor{grey1} \textbf{User-friendly resources} & Tailored for those without a security background. & & 17 & 8 \\
%   & \textbf{Tooling recommendations} & The ability to provide feedback and make report adjustments. & & &  \\
   & \textbf{Gamification for projects} & E.g., a green shield for projects with proper PSFs set up. & \cite{moldon2021gamification,trockman2018adding,dabbish2012social} & 13 & 6 \\
   & \rowcolor{grey1} \textbf{PSF checklist} & To-do list for enabling easily configurable PSFs. &  & 15 & 3 \\   
   & \textbf{Nudges or reminders} & Nudges reminding maintainers to consider using PSFs. & & 12 & 5 \\
%   & \rowcolor{grey1} \textbf{Dependency inspection} & Comments and messaging are available during the review process. &  & &  \\
%   & \rowcolor{grey1} \textbf{Auto-merge configurations} & Streamlined and assisted process of creating CVEs. & & &  \\
  \bottomrule
 \end{tabular}
 \end{adjustbox}
 \caption{\codenums factors and tooling codes, shortened to preserve space, identified from the listing survey study and interview study divided into five categories as a result of software vulnerability management efforts. Acronyms listed represent, respectively: platform security features (\textbf{PSF}), existing related work (\textbf{RW}), the number of listing (\textbf{L}) survey study mentions ($n_1=80$), and the number of interview (\textbf{I}) study mentions  ($n_2=22$). The extended table without omitted codes can be found in~\autoref{sec:fulltable}.}
    \label{tab:bigasstable}
 %\end{centering}
 \end{table*}
